Visual Recognition of Great Ape Behaviours in the Wild

We propose a first great ape-specific visual behaviour recognition system utilising deep learning that is capable of detecting nine core ape behaviours.

==> motivations.tex <==


% Motivations include automating a large workload for ecologists
Beyond the archive, there is a vast amount of sensory data that is continuously being documented in the wild. To process all of this manually would take too long, affecting the duration of vital field studies that depend on the data. Automating this would save ecologists a significant amount of time, allowing them to increase their study sizes for more ambitious experiments. It can also help to increase publication rate and contribution to academia. Furthermore, this approach can produce standardised results by removing human bias, leading to better comparisons across experiments and results.

Questions of ethical issues have been raised with regards to field experiments involving great apes. For example, the use of invasive techniques, such as “habituation”, where researchers make the apes acclimatise to them through food provisioning, can be seen as an unwanted interference of a great ape’s growth and development~\cite{greatapeethics}. The mere presence of humans may cause stress among the apes. This is undesirable in itself and in terms of how it may affect the behaviour of apes that are being observed. A non-invasive system can address these issues, taking into consideration the great apes’ health and as a result, producing more reliable results.
